Nonlinear dynamic analysis of an epidemiological model for COVID-19 including public behavior and government action

This paper is concerned with nonlinear modeling and analysis of the COVID-19 pandemic currently ravaging the planet. There are two objectives: to arrive at an appropriate model that captures the collected data faithfully, and to use that as a basis to explore the nonlinear behavior. We use a nonlinear SEIR (Susceptible, Exposed, Infectious & Removed) transmission model with added behavioral and government policy dynamics. We develop a genetic algorithm technique to identify key model parameters employing COVID19 data from South Korea. Stability, bifurcations and dynamic behavior are analyzed. Parametric analysis reveals conditions for sustained epidemic equilibria to occur. This work points to the value of nonlinear dynamic analysis in pandemic modeling and demonstrates the dramatic influence of social and government behavior on disease dynamics.

==> mymargin.tex <==
% margins of 1.25" on sides, and 1" at top and bottom

\setlength{\parindent}{0.0in}
\setlength{\parskip}{2ex}
\setlength{\headsep}{0.25in}
\setlength{\topmargin}{0.0in}
\setlength{\textheight}{8.5in}
\setlength{\textwidth}{6.0in}
\setlength{\oddsidemargin}{0.25in}
\setlength{\evensidemargin}{0.25in}



==> nomenclature.tex <==
% nomenclature.tex



==> references.tex <==
% references.tex

\begin{thebibliography}{00}

%Thiel, M., Romano, C.M., Kurths, J.: Spurious structures in recurrence plots induced by embedding.
%\newblock Nonlinear Dyn. \textbf{44}, 299--305 (2006)

\bibitem{Lin2020} Lin, Q., Zhao, S., Gao, D., Lou, Y., Yang, S., Musa, S., Wang, M.H., Cai, Y., Wang, W., Yang, L., He, D.: A conceptual model for the coronavirus disease 2019 (COVID-19) outbreak in Wuhan, China with individual reaction and governmental action. \newblock International Journal of Infectious Diseases, \textbf{93}, 211-216 (2020).
\bibitem{Yi2009}Yi, N., Zhang, Q., Mao, K., Yang, D., Li, Q.: Analysis and control of an SEIR epidemic system with nonlinear transmission rate. \newblock Mathematical and Computer Modelling,
\textbf{50}(9-10), 1498-1513 (2009).
\bibitem {He2013}He, D., Dushoff, J., Day, T., Ma, J., Earn, D.J.:Inferring the causes of the three waves of the 1918 influenza pandemic in England and Wales. \newblock Proc R Soc B: Biol Sci, \textbf{280}, 20131345(2013)

\end{thebibliography}


==> review.tex <==
 Specific to Coronoavirus: Read2020, Liu2020, Liu2020a, Tang2020, Backer2020, Rocklov2020 (diamond princess), WHO2020, Li2020, Burke2020, Kucharski2020 (good), Wu2020 (good)
Ferguson2020 - Imperial College report

Nonlinear dynamics focus

Hethcote1981 nonlinear dynamics
Earn1998 chaos and synchrony
Schwartz1983 subharmonic bifurcation
Martcheva2015 (book)
Olsen1988 Montecarlo simulation, SEIR, chaos
Nakamura2019 Hamiltonian dynamics
Yan2014 Hopf bifurcation

Kermack1927 - original model
Heesterbeek2015 - review paper
Bauch2003
Hethcote1990 nonlinear incidence
Li2018 comparison
Wang2017 behavioral dynamics with vaccination
Ferguson2006 - comprehensive paper
Yuan2013 nonconstant steady state SI model
Wang2013 media included in sir model.  stochastic diff eq
Li2014  - SIR model with contact transmission.  Good model to use for us?
LiM2014 - delays
Cui2014  - SIRS model with media coverage
Huow014 - malaria
Rao2014 - stochastic perturbation of SIR model
Wang2014  - discrete model
Zhang2014 - cholera traveling wave
Goufo2014 - fractional derivative
Tian2014 - traveling wave
Li2015 - stochastic model (good)
Li2017 - very good paper

Lloyd2007 - network model
Zhao2014 - complex network model
Pastor-Satorras2015 - network model
Chen2017 - contagion model



==> seir.tex <==
% seir.tex

%I am adapting a lot of this from \cite{Martcheva2015}.

\section{SEIR Model}

\cite{Anderson1991}

This includes a state for the exposed class as well, who have the pathogen, but are not infectious.  The new parameter, $\sigma$ is the reciprocal of the latent period.

\ba
\dt{S} & = & \mu -\beta{SI} - \mu S \\
\dt{E} & = &\beta{SI}-\sigma E  - \mu E\\
\dt{I} & = &\sigma E- \gamma I - \mu I \\
\dt{R} & = & \gamma I - \mu R
\ea

An example simulation is shown in \figref{SEIR1} with $S_0=0.9, \beta=1.5, \gamma=0.2, \mu=1/70, \sigma=1/3$.

\epsfigure{figures}{SEIR1}{5.0in}{!}{Response with SEIR model}


